The Marginal Value of Momentum for Small Learning Rate SGD

Momentum is known to accelerate the convergence of gradient descent in strongly convex settings without stochastic gradient noise. In stochastic optimization, such as training neural networks, folklore suggests that momentum may help deep learning optimization by reducing the variance of the stochastic gradient update, but previous theoretical analyses do not find momentum to offer any provable acceleration. Theoretical results in this paper clarify the role of momentum in stochastic settings where the learning rate is small and gradient noise is the dominant source of instability, suggesting that SGD with and without momentum behave similarly in the short and long time horizons. Experiments show that momentum indeed has limited benefits for both optimization and generalization in practical training regimes where the optimal learning rate is not very large, including small- to medium-batch training from scratch on ImageNet and fine-tuning language models on downstream tasks.

==> sections-ICLR/SMDE-p12.tex <==

\subsection{Stochastic Differential Equation Results for SGDM}

\subsection{$\alpha\geq 1$}
When $\alpha=1$, the dynamics $\vx_k$ of SGDM  order-$1$ weakly approximated by $\bvx_{\eta k}$ where
\begin{align} 
\dd{\bvx_t} & = - \bvm_t \dd t\\
\dd{\bvm_t} & = - \lambda \bvm_t \dd t + \lambda\nabla\Loss(\bvx_t)\dd t + \lambda\Sigma^{1/2}(\bvx_t)\dd W_t
\end{align}
When $\alpha>1$, the dynamics $\vx_k$ has following facts:
\paragraph{Fact 1} The SGDM $\vx_k$ is an order-$(\alpha-1)$ weak approximation of 
\[\barvx_k = \vx_0 - \sum_{i=1}^k \eta_i m_0\] 
for steps $k=O(1/\eta)$.

\paragraph{Fact 2} The SGDM $\vx_k$ is an order-$(\alpha-1)/2$ weak approximation of $\bvx_t$. 
\begin{align} 
\dd{\bvx_t} & = - \bvm_t \dd t\\
\dd{\bvm_t} & = \lambda\nabla\Loss(\bvx_t)\dd t + \lambda\Sigma^{1/2}(\bvx_t)\dd W_t
\end{align}
with time scaling $t=\eta^{(\alpha+1)/2}k$ for steps $k=O(\eta^{-(\alpha+1)/2})$.

Consider a 1-dimensional example with $\Loss(x)=\frac{1}{2} ax^2$. The SGDM updates like
\begin{align*}
    \left(\begin{matrix} x_{k+1}\\ m_{k+1} \end{matrix}\right) = \left(\begin{matrix} 1-\eta(1-\beta)a & -\eta\beta\\ (1-\beta)a & \beta \end{matrix}\right)\left(\begin{matrix} x_{k}\\ m_{k} \end{matrix}\right) + \left(\begin{matrix}-\eta\\ 1 \end{matrix}\right) (1-\beta)\sigma v_k
\end{align*}
Let $\kappa=\frac{1}{2}(1+\beta-a\eta(1-\beta))$.
The matrix have eigenvalues
\[\lambda = \kappa\pm\sqrt{\kappa^2-\beta}.\]
$\kappa\sim 1-O(\eta^\alpha)$, $\kappa^2-\beta\sim -O(\eta^{1+\alpha})$
